Direct top-quark decay width measurement in the $t\bar{t}$ lepton+jets channel at $\sqrt{s}$=8 TeV with the ATLAS experiment

This paper presents a direct measurement of the decay width of the top quark using $t\bar{t}$ events in the lepton+jets final state. The data sample was collected by the ATLAS detector at the LHC in proton-proton collisions at a centre-of-mass energy of 8 TeV and corresponds to an integrated luminosity of 20.2 fb$^{-1}$. The decay width of the top quark is measured using a template fit to distributions of kinematic observables associated with the hadronically and semileptonically decaying top quarks. The result, $\Gamma_t = 1.76 \pm 0.33 (\rm{stat.}) ^{+0.79}_{-0.68} (\rm{syst.})\; \rm{GeV}$ for a top-quark mass of 172.5 GeV, is consistent with the prediction of the Standard Model.

==> paper_topwidth_aux.tex <==
\clearpage
\part*{Auxiliary material}
\addcontentsline{toc}{part}{Auxiliary material}


\begin{figure}[!hb]
\begin{center} 
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/LeptonPt_1excl_el_4jets_LLCut.pdf}
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/bJetPt1_1excl_el_4jets_LLCut.pdf}\\
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/LeptonEta_1excl_el_4jets_LLCut.pdf}
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/bJetEta1_1excl_el_4jets_LLCut.pdf}\\
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/MET_et_1excl_el_4jets_LLCut.pdf}
        \includegraphics[width=60mm]{figures/ControlPlots/4jets/Mtw_1excl_el_4jets_LLCut.pdf}
	\caption{Distributions of the lepton and leading $b$-tagged jet \pt, lepton and leading $b$-tagged jet $\eta$, \met and 
	$m^W_{\text{T}}$ in the  
	electron+jets channel for events with exactly one $b$-tagged jet after the event selection.  
	The hatched bands show the normalisation 
	uncertainty on the signal and background contributions and the signal model systematic uncertainties. The first and last bins contain 
	underflow and overflow events, respectively.}
\label{fig:control_plots_el_1excl}
\end{center}
\end{figure}


\begin{figure}[!hb]
\begin{center} 
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/LeptonPt_1excl_mu_4jets_LLCut.pdf}
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/bJetPt1_1excl_mu_4jets_LLCut.pdf}\\
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/LeptonEta_1excl_mu_4jets_LLCut.pdf}
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/bJetEta1_1excl_mu_4jets_LLCut.pdf}\\
	\includegraphics[width=60mm]{figures/ControlPlots/4jets/MET_et_1excl_mu_4jets_LLCut.pdf}
        \includegraphics[width=60mm]{figures/ControlPlots/4jets/Mtw_1excl_mu_4jets_LLCut.pdf}
	\caption{Distributions of the lepton and leading $b$-tagged jet \pt, lepton and leading $b$-tagged jet $\eta$, \met and 
	$m^W_{\text{T}}$ in the  
	muon+jets channel for events with exactly one $b$-tagged jet after the event selection. 
	The hatched bands show the normalisation 
	uncertainty on the signal and background contributions and the signal model systematic uncertainties. The first and last bins contain 
	underflow and overflow events, respectively.}
\label{fig:control_plots_mu_1excl}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\begin{center} 
	\includegraphics[width=70mm]{figures/templatePlots/plot_paper_sigonly_mlb_110404_4jflLL_el_2incl.pdf}
        \includegraphics[width=70mm]{figures/templatePlots/plot_paper_sigonly_bsdR_110404_4jflLL_el_2incl.pdf}
	\caption{Templates for \mlb and \bsdR in the range $0.7 \leq \Gamma_t \leq 3.0$~GeV in the  electron+jets channel for events with $\geq 2$~$b$-tags in the $|\eta| > 1$ region. The lower panel shows the ratio of the templates with varied $\Gamma_t$ to the nominal template generated for a decay width of $\Gamma_t = 1.33$~GeV.}
\label{fig:width_templates_example}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\begin{center} 
	\includegraphics[width=70mm]{figures/templatePlots/plot_paper_sigonly_mlb_110404_4jfsLL_el_2incl.pdf}
        \includegraphics[width=70mm]{figures/templatePlots/plot_paper_sigonly_bsdR_110404_4jfsLL_el_2incl.pdf}
	\caption{Templates for \mlb and \bsdR in the range $0.7 \leq \Gamma_t \leq 3.0$~GeV in the  electron+jets channel for events with $\geq 2$~$b$-tags in the $|\eta| \leq 1$ region. The lower panel shows the ratio of the templates with varied $\Gamma_t$ to the nominal template generated for a decay width of $\Gamma_t = 1.33$~GeV.}
\label{fig:width_templates_example2}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\begin{center} 
	\includegraphics[width=70mm]{figures/templatePlots/plot_paper_sigonly_mlb_110404_4jfsLL_mu_2incl.pdf}
        \includegraphics[width=70mm]{figures/templatePlots/plot_paper_sigonly_bsdR_110404_4jfsLL_mu_2incl.pdf}
	\caption{Templates for \mlb and \bsdR in the range $0.7 \leq \Gamma_t \leq 3.0$~GeV in the  muon+jets channel for events with $\geq 2$~$b$-tags in the $|\eta| \leq 1$ region. The lower panel shows the ratio of the templates with varied $\Gamma_t$ to the nominal template generated for a decay width of $\Gamma_t = 1.33$~GeV.}
\label{fig:width_templates_example3}
\end{center}
\end{figure}



\begin{figure}[!h]
\begin{center}
	\subfloat[]{
         \includegraphics[width=145mm]{figures/PostFit/mlb_prefit_divideall_data.pdf} }\\
	\subfloat[]{
         \includegraphics[width=145mm]{figures/PostFit/bsdR_prefit_divideall_data.pdf} }
         \caption{Pre-fit  distributions based on the nominal templates with $\Gamma_t = 1.33$~GeV for (a) $m_{\ell b}$ and (b) \bsdR. The background contributions are combined. 
	 The lower panel shows the ratio of data over the expected $t\bar{t}$ signal and background. 
	 The eight analysis regions 
	 corresponding to different $b$-tag multiplicity and jet pseudorapidity are shown.
	The vertical lines show the boundaries between the binned variables in different lepton and $b$-tag regions. 
	The hatched band shows the total uncertainty. The systematic uncertainties are calculated bin-by-bin based on the systematic variations by adding differences quadratically. Then, statistical and systematic uncertainties are added quadratically to obtain the quoted total uncertainty.}
		\label{fig:pre_fit}
\end{center}
\end{figure}

\begin{figure}[!hbpt]
\begin{center} 
	\includegraphics[width=90mm]{figures/results/scan_data0_newplot_all.pdf}
	\caption{Twice the negative logarithm of the likelihood obtained from the binned likelihood template fit to data. The full range of likelihood points is plotted.
	The quadratic fit around the minimum as shown in Fig.~\ref{fig:likelihoodScan} is given as well.} 
\label{fig:likelihoodScanFull}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\begin{center}
         \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_1excl_el_4jfsLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_1excl_mu_4jfsLL.pdf}\\
	 \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_1excl_el_4jflLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_1excl_mu_4jflLL.pdf}\\
	 \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_2incl_el_4jfsLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_2incl_mu_4jfsLL.pdf}\\
	 \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_2incl_el_4jflLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_mlb_postfit_2incl_mu_4jflLL.pdf}\\
         \caption{Post-fit distributions of the eight analysis regions plotted separately based on the best-fit templates for $m_{\ell b}$. The background contributions 
	 are combined. The lower panel shows the ratio of data over post-fit $t\bar{t}$~signal and background. The hatched band shows the total uncertainty. The systematic uncertainties are calculated bin-by-bin based on the systematic variations by adding differences quadratically. Then, statistical and systematic uncertainties are added quadratically to obtain the quoted total uncertainty.}
	\label{fig:post_fit_mlb}
\end{center}
\end{figure}


\begin{figure}[!htbp]
\begin{center}
         \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_1excl_el_4jfsLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_1excl_mu_4jfsLL.pdf}\\
	 \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_1excl_el_4jflLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_1excl_mu_4jflLL.pdf}\\
	 \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_2incl_el_4jfsLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_2incl_mu_4jfsLL.pdf}\\
	 \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_2incl_el_4jflLL.pdf}
         \includegraphics[width=54mm]{figures/PostFit/reco_bsdR_postfit_2incl_mu_4jflLL.pdf}\\
         \caption{Post-fit distributions of the eight analysis regions plotted separately based on the best-fit templates for \bsdR. The background contributions 
	 are combined. The lower panel shows the ratio of data over post-fit $t\bar{t}$~signal and background. The hatched band shows the total uncertainty. The systematic uncertainties are calculated bin-by-bin based on the systematic variations by adding differences quadratically. Then, statistical and systematic uncertainties are added quadratically to obtain the quoted total uncertainty.}
	\label{fig:post_fit_bsdR}
\end{center}
\end{figure}




